Born-Infeld Action in String Theory

In this thesis I present applications of the Born-Infeld action to the description of D-branes, mostly in the context of type IIB string theory. First I present the Callan-Maldacena construction of a fundamental string attached to a threebrane, whereby the string is made out of the wrapped brane. This interpretation withstands a rather detailed scrutiny, including the magnitude of the static tension and of the B-I charge; and Polchinski's mixed Dirichlet/Neumann boundary conditions for small perturbations of the string. The latter arise dynamically from the full non-linear equations of motion. Also, the Born-Infeld charge is shown to produce the correct form of dipole radiation under the influence of harmonic oscillations of the string. The second part comprises of the application of these ideas to the AdS/CFT correspondence. Using the essentially non-perturbative nature of the B-I action we were able to construct in the near-horizon geometry of N D3-branes the color-singlet baryon vertex of the SU(N) gauge theory as a fivebrane wrapped on the $S^5$ sphere, with B-I strings playing the role of the quarks. Also, in the asymptotically flat background we obtain a smooth classical description of the Hanany-Witten phenomenon. In the case of non-extremal background we construct baryons of the three-dimensional non-supersymmetric theory, the low energy dynamics of which was conjectured to be equivalent to ordinary QCD. Our approach allows to exhibit confining properties of color flux tubes, i.e. the dependence of the tension of the flux tube on its color content. We do this by building an extended baryon, where a fraction $\nu$ of the total of N quarks is removed to a finite distance.

==> INCLUDE/alb_bib.tex <==
\bibitem{Imamura}
Y.~Imamura, ``Supersymmetries and BPS Configurations on Anti-de Sitter Space,''
\href{http://xxx.lanl.gov/abs/hep-th/9807179}{{\tt hep-th/9807179}}.

\bibitem{cm}
C.~Callan and J.~Maldacena, ``Brane Dynamics from the Born-Infeld Action,'' 
Nucl.~Phys. {\bf B513} (1998) 198, \href{http://xxx.lanl.gov/abs/hep-th/9708147}
{{\tt  hep-th/9708147}}.

\bibitem{gibbons}
G.~Gibbons, ``Born-Infeld Particles and Dirichlet p-branes'',
Nucl.~Phys. {\bf B514} (1998) 603, \href{http://xxx.lanl.gov/abs/hep-th/9709027}
{{\tt  hep-th/9709027}}.

\bibitem{jthroat}
J.~Maldacena, ``The Large N Limit of Superconformal Field Theories and
  Supergravity,'' \href{http://xxx.lanl.gov/abs/hep-th/9711200}{{\tt
  hep-th/9711200}}.

\bibitem{gkpads}
S.~S. Gubser, I.~R. Klebanov, and A.~M. Polyakov, ``Gauge Theory Correlators
  from Noncritical String Theory,'' Phys.~Lett. {\bf B428} (1998) 105,
  \href{http://xxx.lanl.gov/abs/hep-th/9802109}{{\tt hep-th/9802109}}.

\bibitem{wittenholo}
E.~Witten, ``Anti-de Sitter Space and Holography,''
  \href{http://xxx.lanl.gov/abs/hep-th/9802150}{{\tt hep-th/9802150}}.

\bibitem{wittenbaryon}
E.~Witten, ``Baryons and Branes in Anti de Sitter Space,''
J.~High Energy Phys. {\bf 07} (1998) 006,
\href{http://xxx.lanl.gov/abs/hep-th/9805112}{{\tt hep-th/9805112}}.

\bibitem{groguri} 
H.~Ooguri and D.~Gross, ``Aspects of Large N Gauge Theory Dynamics as 
seen by String theory,''
\href{http://xxx.lanl.gov/abs/hep-th/9805129}{{\tt hep-th/9805129}}.

\bibitem{baryonsugra}
A.~Brandhuber, N.~Itzhaki, J.~Sonnenschein, and S.~Yankielowicz,
``Baryons from Supergravity,''
\href{http://xxx.lanl.gov/abs/hep-th/9806158}{{\tt hep-th/9806158}};\\
Y.~Imamura, ``Baryon Mass and Phase Transitions in Large N Gauge 
Theory,''
\href{http://xxx.lanl.gov/abs/hep-th/9806162}{{\tt hep-th/9806162}}.

\bibitem{hw}
A.~Hanany and E.~Witten, ``Type IIB superstrings, BPS Monopoles, and 
Three-dimensional Gauge Dynamics,''
Nucl.~Phys. {\bf B492} (1997) 152,
\href{http://xxx.lanl.gov/abs/hep-th/9611230}{{\tt hep-th/9611230}}.

\bibitem{bdg}
C.~P.~Bachas, M.~R.~Douglas, and M.~B.~Green, ``Anomalous Creation of
Branes,'' J.~High Energy Phys. {\bf 07} (1997) 002,
\href{http://xxx.lanl.gov/abs/hep-th/9705074}{{\tt hep-th/9705074}}.

\bibitem{dfk}
U.~Danielsson, G.~Ferretti, and I.~Klebanov, ``Creation of 
Fundamental Strings by Crossing D-branes,''
Phys.~Rev.~Lett. {\bf 79} (1997) 1984,
\href{http://xxx.lanl.gov/abs/hep-th/9705084}{{\tt hep-th/9705084}}.

\bibitem{susswi}
L.~Susskind and E.~Witten, ``The Holographic Bound in Anti-de Sitter
Space,''
\href{http://xxx.lanl.gov/abs/hep-th/9805114}{{\tt hep-th/9805114}}.

\bibitem{pp}
A.~W.~Peet and J.~Polchinski, ``UV/IR Relations in AdS Dynamics,''
\href{http://xxx.lanl.gov/abs/hep-th/9809022}{{\tt hep-th/9809022}}.

\bibitem{emp}
R.~Empar\'an, ``Born-Infeld Strings Tunneling to D-branes,''
Phys.~Lett. {\bf B423} (1998) 71,
\href{http://xxx.lanl.gov/abs/hep-th/9711106}{{\tt hep-th/9711106}}.

\bibitem{wittenthermo}
E.~Witten, ``Anti-de Sitter Space, Thermal Phase Transition, and
Confinement in Gauge Theories,''
Adv.~Theor. Math.~Phys. {\bf 2} (1998) 505,
\href{http://xxx.lanl.gov/abs/hep-th/9803131}{{\tt hep-th/9803131}}.

\bibitem{aki}
A.~Hashimoto, ``The Shape of Branes Pulled by Strings,''
\href{http://xxx.lanl.gov/abs/hep-th/9711097}{{\tt hep-th/9711097}}.

==> INCLUDE/intro_old.tex <==
Research into various aspects of D-branes in the past few years
has become synonymous with the New String Theory. Beginning 
with the first work by Dai, Leigh and Polchinski in 1989 \cite{pol},
and the key discovery by Polchinski \cite{rr} of the fact that D-branes carry
RR charges led to an incredible amount of activity surrounding branes.
D-branes, in particular the D2-brane and the NS5-brane are presently 
thought to be the fundamental objects of M-theory, which is conjectured
to incorporate all the known species of string theory, plus the 
11-dimensional supergravity. An important milestone was the 
construction of the corresponding supergravity solutions by
G.~Horowitz and A.~Strominger \cite{stroho}.
This work itself built on the previous construction of the SUGRA 
solution for an infinite fundamental string by Dabholkar and Harvey 
\cite{daha}.

The Born-Infeld action, sometimes also referred to as Dirac-Born-Infeld
action is the effective action for low-energy degrees of freedom of the
D-brane \cite{leigh}. The consistency of the $\sigma$-model for the world-sheet
of the string is shown there to require that the brane be described by BI action,
just like in the general curved background requiring consistency of string theory
leads to the Einstein-Hilbert action. It should come as no surprise then, 
that BI is also invariant under general coordinate transformations,
in fact it can be thougth as a theory with a more general metric, where the
anti-symmetric part of the metric tensor is identified with the electromagnetic field.
This was the thinking of Born and Infeld \cite{bi} when they presented the final
version of their modified electrodynamics. The original motivation was to
get a better behaved theory, one that would not have the Coulomb self-energy
divergence, etc... Also one might hope that the corresponding quantum
field theory might be better behaved too, but progress is of course 
hindered by the fact that the action contains an infinite number of 
unrenormalisable interactions.
 
As explained above, the key difference with 
previously known p-branes and supermembranes 
\cite{supermembrane,supermembrane1,supermembrane2} is the inclusion
of a worldvolume electromagnetic field. This field corresponds on the 
string theory side to virtual states of an open string, where both
ends are fixed to move in the worldvolume of the brane.

The starting point for this thesis is the paper by Callan and
Maldacena \cite{cm}, hereafter referred to as CM.
They, noting that most treatments of D-branes were done using
the linearized theory, undertook to fully account  for the
specific non-linearities of the Born-Infeld
{\it super-electrodynamics}. The static features of 
intersecting branes are determined by SUSY and BPS arguments,
however dynamical issues have to be explored using the full 
Born-Infeld action. They construct, first and foremost, the 
 solution for a fundamental string ending on a D-brane, in which
the junction-point of the string manifests itself as a point Coulomb charge
in the world-volume of the brane. They also find a non-BPS solution
corresponding to a brane and an anti-brane joined by e.g. a
fundamental string.

This thesis is based on a series of papers that arose directly
out of the approach Callan and Maldacena took in their paper.
For the sake of convenience I list these papers in the order in which they
are presented in this thesis:
\begin{itemize}
\item ``Neumann Boundary Conditions from Born-Infeld Dynamics,''\\
by K. Savvidy, G. Savvidy, {{\tt hep-th/9902197}}
\item ``Brane Death via Born-Infeld String'', by K. Savvidy, {{\tt hep-th/9810163}} 
\item ``Baryons and String Creation from the Fivebrane Worldvolume Action,''\\ 
by C.G. Callan, A. Guijosa, K. G. Savvidy, {{\tt hep-th/9810092}}
\item ``Baryons and Flux Tubes in Confining Gauge Theories from Brane Actions,''\\
by C.G. Callan, A. Guijosa, K. G. Savvidy, O. Tafjord, {{\tt hep-th/9902197}} 
\end{itemize}
I have used the texts of these papers to large extent verbatim,
especially in the case of the latter two papers, in this thesis.

In Chapter 1 I review some general facts about the Born-Infeld action.
In particular, section \ref{gen_cov} deals with the two possible representations
of the action, the manifestly generally covariant one, and the dimensionally
reduced version which is necessarily in the "static" gauge. Section 
\ref{nonabelian} discusses briefly the subject that hasn't received full 
development as yet, that of non-Abelian generalization of the B-I action.

In Chapter 2 I present some applications of ideas from CM to 
threebrane physics. Specifically, sections \ref{dirichlet} and \ref{neumann}
show how Polchinski's open string boundary conditions arise dynamically
from the B-I  treatment of the F-string attached to a D3-brane. 
In CM it was shown that
excitations which are normal to both the string and the 3-brane behave as if
they had Dirichlet boundary conditions at the point of attachement.
We show that certain excitations of the F-string/D3-brane 
system can be shown to obey   Neumann boundary conditions by considering 
the Born-Infeld dynamics of the F-string (viewed as a 3-brane cylindrically
wrapped on an $S_2$). In CM it was shown that
excitations which are normal to both the string and the 3-brane behave as if
they had Dirichlet boundary conditions at the point of attachment. 
In \cite{neumannP} 
we show that excitations which are coming down the string with a 
polarization along a direction parallel to the brane are almost completely
reflected just as in the case of all-normal excitations, but the end of
the string moves freely on the 3-brane, thus realizing Polchinski's
open string    Neumann
boundary condition dynamically. In the low energy limit 
$ \omega \rightarrow 0$, i.e. for wavelengths much larger than the string
scale only a small fraction $ \sim \omega^4$ of the energy escapes in
the form of dipole radiation.
The physical interpretation is that a string attached to the 3-brane 
manifests itself as an electric charge, and waves on the string cause
the end point of the string to freely oscillate and therefore produce 
electromagnetic dipole radiation in the asymptotic outer region.

Section \ref{brane_death} contains the calculation of the brane-anti-brane
potential, which can be used to capture some new features of the quasi-classical 
tunneling of the brane-anti-brane pair joined by an F-string. This is
of relevance to a subject that has since attracted certain attention,
the brane-anti-brane annihilation: see e.g. A.~Sen, "Tachyon condensation.." 
and E.~Witten "D-branes and K-theory". Our calculation shows that for 
a distance between the branes that is larger than some critical distance,
determined by the string coupling, the stretched string is indeed quasi-stable,
while for shorter distances it is tachyonic.

The attraction between
the branes causes them to approach and at some point to tunnel, 
because the action of the bounce solution goes to zero.
The energy of the solution at the top of the barrier, the sphaleron, goes like
$\sim D^3$ for large separations D, while the energy of the string is proportional
to its length D. 


Chapter 3 has a slightly different flavor. There, the B-I action
is used to describe a fivebrane placed in the supergravity background
of N coincident D3-branes. In the near-horizon limit, according to Witten,
the background five-form RR field induces N units of electric charge
on the fivebrane, which should be interpreted as N fundamental strings
attached to it. These strings play the role of quarks in the AdS/CFT correspondence,
and the configuration as a whole is interpreted as a color neutral baryon
of SU(N) {\it super}-YM theory.

In essence, B-I is known to incorporate corrections to string theory to all
orders in $\ap$, and thus allows us to construct an essentially non-perturbative
object on the gauge theory side: the baryon. In addition, this approach is
self consistent, since B-I action is only valid for slowly varying fields
(the action does not contain derivative-dependent corrections to the effective string
action). Our solutions  have fields that are everywhere smooth thus
ensuring the consistency of our description.

The extension of these to the full D3 metric results in a nice 
classical description of the Hanany-Witten phenomenon, whereby strings are
created when a flat D5-brane is pulled through the threebrane stack.
A surprising byproduct is the configuration where N/2 strings are stretched 
to the threebranes on either side, and change their orientation when one
crosses the threebrane. Thus the total change in the number of strings
is N, as expected. This configuration%
\footnote{It was found for the case of 0-brane in \cite{dfk}.},
is characterized by zero force on the 5-brane, as the attraction due to the
tension of the string is exactly balanced by electrostatic repulsion. 
These considerations
seem to suggest the actual existence of the 1/2 string state, the proper
interpretation of which is at present not clear.

In the section \ref{3dsec} we use near-horizon geometry
of non-extremal D3-branes to find embeddings of a D5-brane which describe
baryonic states in three-dimensional QCD.
In particular, we
construct solutions corresponding to a baryon made of $N$ quarks,
and study what happens when some fraction $\nu$ of the total
number of quarks are bodily moved to a large spatial separation
from the others. The individual clumps of quarks are represented
by Born-Infeld string tubes obtained from a D5-brane whose
spatial section has topology ${\bf R}\times {\bf S}^4$.
They are connected by a confining color flux tube, described
by a portion of the fivebrane that runs very close and parallel
to the horizon. We find that this flux tube has a tension with a
nontrivial $\nu$-dependence (not previously obtained by other methods).
We also discuss related questions including binding energies,
string creation, and the appearance of new energy scales.



==> INCLUDE/nonextr.tex <==


We consider\footnote{This section is based on the recent paper \cite{nonextrP}
by C.G. Callan, A.Guijosa, O.Tafjord and myself.}
Wilson loops of QCD-3 in non-extremal AdS background, 
which correspond
to a baryon made out of N quarks, where a fraction $\nu < 1$ of those 
is removed to a finite (or infinite) separation. We model this by 
considering a D5-brane with Born-Infeld action. In this picture the quarks
are made of a fivebrane wrapped on $S_4$, where the number of quarks is 
determined by tension of the resulting tube. The color flux tube is also
made of a wrapped fivebrane which runs very close and parallel to the 
horizon. The tension of the color flux tube is proportional to 
the square of the radius of the horizon $r_0^2$, times a factor
determined by $\nu$. Thus we obtain the dependence of the flux tube tension 
on its color content. This dependence is non-trivial and has not been 
obtained by other methods.

Our approach is an extension of the previous paper \cite{baryon}
(see also \cite{imamura}) in which Born-Infeld approach to 
constructing strings out of Dbranes \cite{cm,gibbons} was used to
build baryons of the four-dimensional SU(N) SYM. This follows recent work
\cite{juan, wittenbaryon, groguri} on the construction of the
large N limit of gauge theories from supergravity in AdS. Wilson loops
on the gauge theory side, constructed through "hanging" strings or branes
were considered in \cite{groguri,rey,baryonsugra}. The key new 
element of our present paper is in the possibility to make not
just mesons, e.g. quark-anti-quark pairs, but SU(N) baryons
in which some number of quarks have been removed to a finite 
distance. 

In our previous paper \cite{baryon} we have obtained D5-brane congfigurations in AdS,
which represent SU(N) baryons. Among the moduli of this solutions is
the parameter $\nu$, the integration constant of the electric field, 
which allowed us to separate the tube with N quarks for $\nu=1$ into 
two tubes, one with $\nu N$ and the other with $(1 - \nu)N$ quarks.
Existence of one of these without the other is not certain, at least
for $\nu \neq 0, 1, 1/2$ , but in this paper we will show how one can 
separate these two quark bundles by finite distance and generate 
tension in the non-extremal background.

\subsection{Equations of motion for the fivebrane}

We will consider the scaling limit of the asymptotically flat
non-extremal background, which is an AdS space with a horizon at $r_0$.
Taking this limit can be thought of as taking $r_0$ to be small compared
to R ( $R^4= 4 \pi g_s N $), and then compactifying time on a small
circle. The resulting theory should have the same dynamics as
three-dimensional QCD
\cite{wittenbaryon} in the strong coupling 
regime at high temperature ($g_{YM}=\sqrt{T}$),
similar to the strong couping regime of lattice QCD. 


The scaling limit of the metric is given by 
\be
ds^2=\frac{r^2}{R^2}(-f dt^2+dx^2+dy^2+dz^2)+
\frac{R^2}{r^2}(f^{-1}dr^2+r^2 d\Omega_5^2),
\label{metric}
\ee
where $f=1- \frac{r_0^4}{r^4}$.
We will henceforth drop R, and set $r_0=1$ without any loss of generality,
and it should be understood that $ r_0 \le r  << R $.

We would like to consider a D5-brane in this background. Since our 
purpose is to evaluate the Wilson loop of QCD-3, we set up the brane
to be infinitely long in the $y$ direction. In the $x$ direction, the brane 
will be stretched to a finite distance and we would like to show that 
the energy is proportional to the distance.

The final picture is that of an $SU(N)$ baryon in which fractions $\nu$ 
and $1- \nu $ of the quarks are separated in the $x$ direction, and are 
connected by a color flux tube running along the horizon.

The world volume of the fivebrane is parametrized by six parameters 
$\tau,~ \sigma_1,~\sigma_2,$$~ \sigma_3,~ \sigma_4$ and $s$. The embedding of this
fivebrane into 10-dimensional target space is defined by

\be 
\begin{array}{ll}
x=x(s),    & \theta_1=\sigma_1, \\
y=\tau,    &\theta_2=\sigma_2,  \\
z=Const=0, &\theta_3=\sigma_3,  \\
t=Const=0, &\theta_4 =\sigma_4, \\
r=r(s),    &\theta_5 = \theta(s),
\label{staticgauge}
\end{array} 
\ee
where only $x$, $\theta_5$ and $r$ are functions of the parameter $s$. 
The coordinate $y$ plays the role of time in this QCD-3. 



The Born-Infeld determinant for this embedding of the fivebrane 
results in the following action
\be
L= T_5 \Omega_4 \int ds~ sin^4\theta(s)~ \sqrt{ r^2~\left[r^2x'(s)^2 + 
\frac{1}{r^2}\left( r^2 \theta'(s)^2 + \frac{r'(s)^2}{f} \right)\right] - B_{\tau s}^2 }~+
(Source Term) 
\ee
\be
(Source Term) = \int F^{(2)} \wedge C^{(4)} = 4 \int  A_{\tau}~ sin^4\theta 
~d\theta~.
\ee
Compare this to the expressions in \cite{baryon} for the extremal case.
The magnetic field of QCD-4 $B_{\tau s}$ is an electric field in QCD-3,
since $y$ is now the time direction.
Just like in the extremal case it is possible to introduce the displacement
$ D={\partial L}/{\partial B}$ and make a Legendre transformation to 
get rid of B. The equation for $D(\theta)$ and its solution are the same as before:
\be
\begin{array}{c}
{dD(\theta) \over d\theta} =-4sin^4\theta\\
D(\theta)= 
\left[{3\over 2}(\nu\pi-\theta) 
  +{3\over 2}\sin\theta\cos\theta+\sin^{3}\theta\cos\theta\right]~,
\label{deqns}
\end{array}
\ee
where the integration constant has been written in terms of a parameter 
$0\le\nu\le1$.

After the Legendre transformation we get an energy function 
\be
U = T_5 \Omega_{4}\int ds 
\sqrt{r^4 x^\prime(s)^2+ r^2\theta^\prime(s)^2 + f^{-1} r^\prime(s)^2}~%
\sqrt{ D^2(\theta) + \sin^8\theta }.
\label{action}
\ee
This functional has complicated root structure which results in
tangled Euler- Lagrange equations. In order to resolve this problem
note that the functional has the residual
reparametrization invariance in $s$, which remained even after fixing all the 
other coordinates in the 
static gauge (\ref{staticgauge}) 
\be
s \rightarrow \phi(s),~~~ x' \rightarrow x'/\phi',~~~r' 
\rightarrow r'/\phi'~~~ \theta' \rightarrow \theta'/\phi'.
\ee
Let us introduce the conjugate momenta to $x$, $r$ and $\theta$, 
\be
p_x=\frac{\partial U}{\partial x^\prime},~~~~~~~p_r=\frac{\partial U}
{\partial r^\prime},~~~~~~~p_\theta=\frac{\partial U}
{\partial \theta^\prime}. \label{momenta}
\ee
The hamiltonian is zero identically, which is the consequence of 
reparametrization invariance and in addition the system should have 
a constraint\footnote{We would like to thank 
G.Savvidy for suggesting and helping to realize this approach.} 
which is not difficult to find from (\ref{momenta}):
\be
\tilde{H} = {1\over2} \left( f p_r^2 + \frac{p_{\theta}^2 }{ r^2} + 
\frac{p_x^2}{r^4}-
\left( D^2(\theta)+sin^8\theta \right) \right).
\label{ham}
\ee
This constraint can be taken as the Hamiltonian and thus 
conveniently fixes the gauge, while getting rid of the 
complicated square-root structure of the action.\\
The equations of motion that follow from this Hamiltonian are:


\be
\begin{array}{ll} 
\dot p_r = \frac{2p_x^2}{r^5}-\frac{2p_r^2 }{r^5}+ \frac{p_\theta^2}{r^3} ,
& \dot r = ( 1-\frac{1}{r^4}) p_r,\\
\dot p_\theta = 4sin^4\theta \left( sin^3\theta cos\theta-D(\theta) \right),& 
\dot\theta=\frac{p_\theta}{r^2}, \\
\dot p_x =0,& \dot x = \frac{p_x}{r^4}.
\label{eqns}
\end{array}
\ee
Together with initial conditions, these equations completely define
the solutions for the fivebrane. The initial conditions should be 
chosen such that $\tilde H=0$.



\subsection{Color dependence of string tension}

We are looking for the solution of these equations with $\nu N$ and $(1-\nu)N$
quarks separated by distance $\vert x(+\infty)-x(-\infty)\vert$. 
The quarks are made of the fivebrane wrapped on $S_4$, with 
tubes pointing in $\theta\rightarrow 0$ and $\theta \rightarrow \pi$ 
directions respectively. The quarks are connected by a flux tube, 
which is made out of a fivebrane running close to the horizon at 
$\theta=\theta_{cr}$. This $\theta_{cr}(\nu)$ is determined from the equation 

$$\pi\nu=\theta_{cr}-\sin\theta_{cr}\cos\theta_{cr}.$$ 
The result is that $\theta_{cr}(\nu)$ is a monotonous function of $\nu$, 
with 
$\theta_{cr}(1)= \pi, ~\theta_{cr}(0) =0$ and 
$\theta_{cr}({1 \over 2}) = \frac{\pi}{2}$.

The initial condition are defined by the equations

\be
\begin{array}{ll} 
r(0)= 1 + \epsilon,&  p_r(0)=0,\\
\theta(0)=\theta_{cr},&  p_{\theta}(0)=\eta,\\
x(0)=0,&  p_x(0)=\sqrt{r^4(0) (D^2(\theta_{cr}) +sin^8\theta_{cr}) -\eta^2 r^2(0)}
\label{inicon}
\end{array} 
\ee
and  are parametrized by $\epsilon$, the distance from the horizon at
the point of closest approach. The parameter $\eta$ is a function of $\epsilon$,
and is determined by the requirement that the solution behave as a straight cylinder
in both $\theta\rightarrow 0$ and $\theta \rightarrow \pi$ limit. 
Indeed, it is natural to require
asymptotically BPS behavior in the region of space (e.g. far from the horizon) 
where supersymmetry is recovered.

\begin{figure}
\centerline{\hbox{\psfig{figure=\path 3d.eps,height=12cm,angle=0}}}
\caption[fig1]{ The 3-dimensional projection of the D5-brane. 
Every point on the curve is a projection of an $S_4 \times R$. 
One can clearly see how the brane comes close,
then extends along the horizon, and finally leaves at the other end. 
From the point of view of the 3-dimensional gauge theory, 
which lives in the x-y-z space, this configuration 
corresponds to a static SU(N) baryon, in which $\nu N$ and $(1-\nu)N$ 
quarks have been separated by a finite distance in the x direction.} 
\label{3deps}
\end{figure}

\begin{figure}
\centerline{\hbox{\psfig{figure=\path zro.eps,height=12cm,angle=0}}}
\caption[fig2]{ The 2-dimensional projection of the D5-brane into 
$z=r cos \theta,~\rho=r sin \theta$ plane. 
Note the similarity in the shape of the branches to the extremal case.
The brane extends itself in the x-direction mostly 
at the inflection point (the cusp), while
x is almost constant at the ends, where the quark tubes are attached. 
The branch pointing up has $\nu N$ quarks, 
while the branch pointing down has $(1-\nu)N$ quarks.
} 
\label{zroeps}
\end{figure}

It is  seen from the equation for $\dot r$ in (\ref{eqns}) that $r-r_0$
grows exponentially with an exponent proportional to $p_r$, which itself 
reaches the value  close to $p_x$ (see equation for $\dot p_r$).
Therefore  the separation between the quarks increases only logarithmically, 
as one gets closer to the horizon\footnote{At the inflection point,
e.g. the point of closest approach to the horizon.}. In fact, there 
exists
a limiting solution which consists of $\nu N$ quarks with a flux tube that
extends to infinity, and the brane approaches the horizon exponentially 
with distance.

In order to obtain the tension of the color flux tube on $\nu$, or 
equivalently on its color content, note that when the fivebrane runs parallel
and close to the horizon, the action {\ref{action}) reduces to 
$\int dx \sqrt{D^2(\theta) + sin^8 \theta } $. Thus, to obtain the tension
explicitly, one needs to evaluate the expression 
$r_0^2/R^2 \sqrt{D^2(\theta_{cr}) + sin^8 \theta_{cr} } $ as a function 
of $\nu$ (see Fig. \ref{tensioneps}). Note that in all cases the tension is proportional 
to $T_5 \Omega_4 r_0^2/R^2$, and vanishes as we approach extremality.

\begin{figure}
\centerline{\hbox{\psfig{figure=\path tension.eps,height=10cm,angle=0}}}
\caption[fig3]{ The tension of the flux tube as a function of the percentage of
the quarks removed. In principle $\nu$ should be quantized in units of ${1 / N}$.
The tension tends to zero as $\nu$ approaches 0 or 1, which } 
\label{tensioneps}
\end{figure}

Let us discuss the tension of the color flux tube qualitatively. 
As one might expect, the tension linearly increases for small $\nu$. This means
that for each additional quark removed the work done is approximately
constant. Also it seems to suggest
that a single quark becomes lesser and lesser bound at large N. There is a
complete symmetry between $\nu$ and $1-\nu$, (e.g. for examlpe it shouldn't
matter whether 1 quark was removed or $N-1$). Thus, tension flattens out
at $\nu=1/2$ and comes back down to zero near $\nu=1$. In QCD language,
the flat part of the curve means that it doesnt cost any energy to move
the quark from one bundle with $\sim N/2$ quarks to the other.






==> INCLUDE/statics_old.tex <==
Research into various aspects of D-branes in the past few years
has become synonimous with the New String Theory. Beginning 
with the first work by Dai, Lee and Polchinski in 1989 \cite{pol},
and the key discovery by Polchinski \cite{rr} of the fact that D-branes carry
RR charges led to an incredible amount of activity surrounding branes.
D-branes, in particular the D2-brane and the NS5-brane are presently 
thought to be the fundamental objects of M-theory, which is conjectured
to incorporate all the known species of string theory, plus the 
11-dimensional supergravity. An important milestone was the 
construction of the corresponding supergravity solutions by
G.~Horowitz and A.~Strominger \cite{stroho}.
This work itself built on the previous construction of the SUGRA 
solution for an infinite fundamental string by Dabholkar and Harvey 
\cite{daha}.

The starting point for this thesis is the paper by Callan and
Maldacena \cite{cm}, hereafter referred to as CM.
They, noting that most treatments of D-branes were done using
the linearized theory, undertook to fully account  for the
specific non-linearities of the Born-Infeld
{\it super-electrodynamics}. The static features of 
intersecting branes are determined by SUSY and BPS arguments,
however dynamical issues have to be explored using the full 
Born-Infeld action. They construct, first and foremost, the 
 solution for a fundamental string ending on a D-brane, in which
the end-point of string manifests itself as a point Coulomb charge
in the world-volume of the rane. They also find a non-BPS solution
correspoding to a brane and an anti-brane joined by e.g. a
fundamental string.

We repeat their arguments for the construction. Starting from
a 10-dimensional B-I action and dimensionally reducing to 3+1
dimensions we need to compute the action
\be
S = - \int d^{4}x
\sqrt{- {\rm {\rm det}} (G_{\mu\nu} + {F}_{\mu\nu})}
\ee
where only one of the 6 available scalars is excited. The actual
determinant that needs to be computed is
\bea
\nonumber
\left[
\mbox{
$\begin{array}{ccccc}
-1  & E_1 & E_2 & E_3 & 0       \\
-E_1& 1   & B_3   & -B_2   &\PD_1\phi\\
-E_2& -B_3   & 1   & B_1   &\PD_2\phi\\
-E_3& B_2   & -B_1    & 1   &\PD_3\phi\\
0   & -\PD_1\phi & -\PD_2\phi & -\PD_3\phi &1
\end{array}$}
\right]\\
=1+ \vec{B}^2 - \vec{E}^2 -\left(\vec{E} \cdot \vec{B} \right)^2 -
   (\partial_0 \phi)^2(1+\vec{B}^2) +(\vec{\partial}\phi)^2\\
   +\left(\vec{B}\cdot \vec{\partial} \phi\right)^2 - 
    \left(\vec{E}\times \vec{\partial}\phi\right)^2+
   2\partial_0 \phi\left(\vec{B}[\vec{\partial} \phi\times\vec{E}]\right)
\nonumber
\eea
This expression was computed by myself  in June 1997,
and a slightly less general version can  be found 
in the review be Gibbons \cite{gibbons}.
In CM supersymmetry analysis is used to find the required solution.
this is possible because for supersymmetric BPS configurations the value
of the B-I action coincides with the linear theory. Thus one can 
find the required solution by constructing one for the linear theory
and then checking that it satisfy the equations of motion of the
full non-linear theory.

{\small

We begin by using BPS arguments to find some solutions of the p-brane
worldsheet gauge theory which have the interpretation of strings ending on 
branes and  D-p branes  ending on D-(p+2)-branes. Let us first assume that the 
massless excitations of a p-brane are described by the dimensional
reduction of the $10$-dimensional  Maxwell action. This ignores important 
nonlinearities (which we will consider later) but will provide a useful 
orientation. The supersymmetry variation of the gaugino is
\be
\label{gauginovar}
{\delta \chi = \Gamma^{\mu\nu} F_{\mu\nu} \epsilon}
\ee
where $\mu\nu$ are ten-dimensional indices. A BPS background is one
where $\delta\chi=0$ for some $\epsilon$. Now imagine we have a point charge 
Coulomb gauge field, or $A_0 = c_p/r^{p-2} $ where $r$ is the spatial 
$p$-dimensional distance and $c_p$ is fixed by some charge quantization 
condition. So far only $F_{0r}\ne 0$ and \ref{gauginovar} shows that there are 
no preserved supersymmetries  since  $\Gamma^{0r}$ has no zero eigenvalues. 
We can, however, also excite one of the transverse scalar fields. Indeed,
$X^9 = c_p/r^{p-2}$ is a solution of the linearized field equation for $X^9$
for which $F_{9r}\equiv \partial_r X^9 = F_{0r}$. In the 
presence of both excitations \ref{gauginovar} reduces to 
\be
\label{preservedsusy}
( \Gamma^{0r} + \Gamma^{9r}) \epsilon = 0~~\Rightarrow~~
(\Gamma^{0} + \Gamma^{9}) \epsilon = 0.
\ee
The usual arguments tell us that half of all choices for $\epsilon$
satisfy this condition. In other words, this background preserves
half the supersymmetries originally possessed by the p-brane and is
still a BPS-saturated state. 

What is the interpretation of such a state? The excitation of the $X^9$ field 
that we have chosen amounts to giving the brane a transverse \lq spike\rq\ 
protruding in the $\hat 9$ direction and running off to infinity. 
It turns out that this spike must be interpreted as a fundamental 
string attached to the D-p-brane. To show this, we calculate the energy of the 
configuration. Of course, the energy of a Coulomb field is strictly infinite,
but let us look at this infinity in more detail by calculating the energy for 
$r \ge \delta $ where $\delta $ is small. We find\footnote{We are 
setting $\alpha' =1$ and using  conventions in which $g \rightarrow 1/g$
under S-duality.}
\be
\label{energy}
E(\delta) = { 1\over (2 \pi)^p g} \int  d^p r  {1\over 2} \{ F_{0r}^2 +
  F_{09}^2  \} = {c_p^2 (p-2)^2 \over  (2 \pi)^p g} 
 \int d^p r {1\over r^{2(p-1)}} =
 {c_p^2 (p-2) \Omega_{p-1}  \over  (2 \pi)^p g}  { 1\over \delta^{p-2}}~,
\ee
where $\Omega_p$ is the volume of the unit $p$-sphere.
Remarkably, this energy is proportional to the value of $X^9$ at $\delta$:
\be
\label{energydelta}
E(\delta) = { c_p  \Omega_{p-1} ( p-2 ) \over (2 \pi)^p g} X^9(\delta)~.
\ee
In the limit $\delta\to 0$ the transverse \lq spike\rq\ is infinitely
long and has infinite energy by virtue of having a constant energy per unit
length. This interprets the Coulomb energy divergence as being due to
an infinitely long string attached to the brane! We should be able to tell 
just what kind of string it is from the value of its energy per unit length. 

Since we expect the source of a worldvolume {\it electric}
field to be the fundamental string, we should be able to see that \ref{energy}
matches the energy per unit length of a fundamental string. To do this,
we need to identify the charge quantization constant $c_p$. Consider first
a 1-brane with (necessarily constant) gauge field $F_{01}$ excited. Depending
on the strength of $F_{01}$, this is a type IIB D-string with 
 some number $n$ of adsorbed fundamental strings. From the BPS mass formula
we know that the tension of such excited strings is $(1/g + g n^2/2)T_f $ for 
small $n$ and string coupling $g$ (where  $T_f = 1/2\pi$ is  the
fundamental string tension).  In the linearized weak field limit of the
BI action the additional tension due to the electric field is 
$(1/2 g) F_{01}^2 T_f $.
This implies that the quantization condition on the one-dimensional electric
field is $F_{01} = g n $. The higher-dimensional cases are related to this by
T-dualities and one can see that the general quantization condition on
the electric flux is
\be
\label{qcond}
{ 1 \over (2 \pi)^{p-1} } \int_{S_{p-1}} F_{0r}  = g n~.
\ee
This implies that $c_p (p-2) \Omega_{p-1}/(2\pi)^{p-1} = g $ 
 and that the energy of the unit charge Coulomb solution is 
\be
\label{energyfinal}
E(\delta) = { 1\over  2 \pi} X^9(\delta) = T_f X^9(\delta)
\ee
This is the energy of a fundamental string of length $X^9(\delta)$.
The analysis works for any value of $p$ and tells
us that there is a BPS gauge configuration describing the attachment of a
fundamental string to {\it any} D-brane. This is exactly what Polchinski's
string theoretic description of D-brane solitons would lead us to expect
\ref{pol_tasi} .

There is one further possibility for solutions of the kind we are discussing.
On a $3+1$-dimensional worldvolume (D3-brane) there exist magnetic point
charge solutions for which $F_{\hat \theta \hat \phi} = N c_m/ r$ (and $c_m$ 
will be determined by magnetic monopole charge quantization conditions)%
\footnote{
Were $\hat \theta,~\hat \phi$ denote unit vectors.}. Taking the 
transverse coordinate excitation to be $X^9 = N c_m/r$, the condition for
unbroken susy now reads
\be
\label{susydstring}
( \Gamma^{\hat \theta \hat \phi} + \Gamma^{9r} ) ~\epsilon =0\qquad{\rm or}\qquad
\Gamma^{1239} ~\epsilon = \epsilon ~.
\ee
This is exactly what we expect for the preserved susy when a type IIB D1-brane 
along $\hat 9$ is attached to a D3-brane along $123$. The energy analysis of 
this solution is consistent with this picture and shows that $c_m =\pi$, 
independent of the string coupling $g$. Among other things, this implies that 
the shape of the solution is independent of the string coupling. 
Clearly the same solution would describe a D-$p$-brane ending on a 
D-$(p+2)$-brane. 

}
